Online Alternating Direction Method (longer version)

Online optimization has emerged as powerful tool in large scale optimization. In this pa- per, we introduce efficient online optimization algorithms based on the alternating direction method (ADM), which can solve online convex optimization under linear constraints where the objective could be non-smooth. We introduce new proof techniques for ADM in the batch setting, which yields a O(1/T) convergence rate for ADM and forms the basis for regret anal- ysis in the online setting. We consider two scenarios in the online setting, based on whether an additional Bregman divergence is needed or not. In both settings, we establish regret bounds for both the objective function as well as constraints violation for general and strongly convex functions. We also consider inexact ADM updates where certain terms are linearized to yield efficient updates and show the stochastic convergence rates. In addition, we briefly discuss that online ADM can be used as projection- free online learning algorithm in some scenarios. Preliminary results are presented to illustrate the performance of the proposed algorithms.

==> conv.tex <==
We now prove the $O(1/T)$ convergence rate for ADM using a variational inequality (VI) based on the Lagrangian given in \myref{eq:lag1}.
%\begin{align}
%\min_{\x \in \mathcal{X},\z \in \mathcal{Z}} \max_{\y} L(\x,\y,\z) = f(\x) + g(\z) + \langle \y, \bA\x + \bB\z - \c \rangle
%\end{align}
Let $\Omega = \cX \times \cZ \times \R^m$. Any $\w^*=(\x^*,\z^*,\y^*) \in \Omega$ solves the original problem in~\myref{eq:admm_pm} optimally if it satisfies the following variational inequality~\cite{fapa03,Nemi:VI,he12:vi}:
\beq
\forall \w \in \Omega~, ~~~h(\w) - h(\w^*)+ \langle \w - \w^*, F(\w^*) \rangle \geq 0~,
\eeq
where
\begin{align*}
F(\w) = \left [ \begin{array}{c}
\bA^T\y \\
\bB^T\y \\
-(\bA \x + \bB \z - \c)
\end{array}
\right ]
\end{align*}
is the gradient of the last term of the Lagrangian, and $h(\w) = f(\x) + g(\z)$. Then, $\tilde{\w}=(\tilde{\x},\tilde{\z},\tilde{\y})$ approximately solves the problem with accuracy $\epsilon$ if it satisfies
\beq
\forall \w \in \Omega~, ~~~ h(\tilde{\w}) - h(\w) + \langle \tilde{\w} - \w, F(\tilde{\w}) \rangle \leq \epsilon~.
\eeq
We show that after $T$ iterations, the average $\bar{\w}_T = \frac{1}{T} \sum_{t=1}^T \w_{t}$, where $\w_t = (\x_t,\z_t,\y_t)$ are from \myref{eq:admm_x}-\myref{eq:admm_y}, satisfies the above inequality with $\epsilon = O(1/T)$.
\begin{thm}
Let $\bar{\w}_T = \frac{1}{T} \sum_{t=1}^T \w_{t}$, where $\w_{t} = (\x_{t},\z_{t},\y_{t})$ from \myref{eq:admm_x}-\myref{eq:admm_y}. Then,
\begin{equation*}
\forall \w \in \Omega, ~~~ h(\bar{\w}_T) - h(\w) + \langle \bar{\w}_T - \w , F(\bar{\w}_T) \rangle \leq O\left(\frac{1}{T}\right)~.
\end{equation*}
\end{thm}
%\input{a-badm}


==> lcrADMM.tex <==

The following theorem shows that both the cumulative objective difference w.r.t.~the optimal and the cumulative norms of the constraints, known as the primal and  dual residuals~\cite{boyd10}, are bounded by constants independent of the number of iterations $T$.
\begin{thm}
Let the sequences $\{\x_t, \z_t,\y_t\}$ be generated by ADM. For any $\x^*,\z^*$ satisfying $\bA\x^* + \bB\z^* = \c$, for any $T$, we have
\begin{align}
&\!\!\sum_{t=0}^T\!\left[\!f(\x_{t+1}) \!+\! g(\z_{t+1}) \!-\! (\!f(\x^*) \!+\! g(\z^*)\!)\!\right]
 \!\leq\! \frac{\lambda_{\max}^{\bB}D_{\z}^2\rho}{2}~,\!\! \label{eq:thm_bobj} \\
& \!\!\!\!\!\!\sum_{t=0}^T \!\!\| \!\bA\x_{t+1} \!\!+\!\! \bB\z_{t+1} \!\!-\!\! \c \!\|_2^2 \!\! + \!\! \| \!\bB\z_{t+1} \!\!-\!\! \bB\z_{t}\! \|_2^2 \!\!\leq \!\!\lambda_{\max}^{\bB}D_\z^2 \!\!+\!\! \frac{D_\y^2}{\rho^2}\!\!~.\!\!\!\!\label{eq:thm_bcst}
\end{align}
\label{thm:bobj}
\end{thm}
\vspace*{-9mm}
%The following theorem shows that the cumulative norms of the constraints, known as the primal and  dual residuals~\cite{boyd10} are bounded by a constant independent of the number of iterations $T$.
%\begin{thm}\label{thm:admcst}
%Let the sequences $\{\x_t, \z_t,\y_t\}$ be generated by ADM. For any $T$, we have
%\begin{align*}
%\sum_{t=0}^T \left [ \| \bA\x_{t+1} \right. & \left. + \bB\z_{t+1} - \c \|_2^2  + \| \bB\z_{t+1} - \bB\z_{t}\|_2^2 \right ] \\
%& \leq \lambda_{\max}^{\bB}D_\z^2 + \frac{D_\y^2}{\rho^2}~.
%\vspace*{-5mm}
%\end{align*}
%\label{thm:bconst}
%\vspace*{-5mm}
%\end{thm}
It is easy to verify that the KKT conditions of the augmented lagrangian \myref{eq:lag1} hold if \myref{eq:thm_bcst} holds. The convergence of equality constraint and primal residual implies the convergence of ADM. A result similar to \myref{eq:thm_bcst} has been shown in~\cite{boyd10}, but our proof is different and self-contained along with \myref{eq:thm_bobj}. Although \myref{eq:thm_bobj} shows that the objective value converges to the optimal value, ${\x_{t+1},\z_{t+1}}$ need not be feasible and the equality constraint is not necessarily satisfied.
%\arindam{We dont need this: It is unclear whether \myref{eq:thm_bobj} and \myref{eq:thm_bcst} together are sufficient to establish a concrete convergence rate.}


==> loadm1.tex <==
We linearize the quadratic term in \myref{eq:oadmm1_x} such that
\begin{align}\label{eq:oadm_x2}
\x_{t+1} &= \underset{\x}{\argmin} \{f_t(\x) +  \langle \bA^T \{  \y_t + \rho(\bA\x_t + \bB\z_t -  \c)\}, \x - \x_t \rangle + \eta B_{\phi}(\x,\x_t)\} ~.
\end{align}
All other updates stay the same. The OIADM1 using \myref{eq:oadm_x2} is presented in Algorithm \ref{alg:loadm1}.

\begin{algorithm*}[tb]
\caption{Online Inexact Alternating Direction Method 1 (OIADM1)}
\label{alg:loadm1}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} $f_{t+1}(\x) + g(\z), \bA,\bB,\c, \rho, \eta, \phi(\x)$
\STATE {\bfseries Initialization:} $\x_0,\z_0,\u_0 = \mathbf{0}$
\FOR{$t=0 \text{ to } T$}
\STATE $\x_{t+1} = \argmin_{\x}~ f_t(\x) +  \langle \bA^T \{  \y_t + \rho(\bA\x_t + \bB\z_t -  \c)\}, \x - \x_t \rangle + \eta B_{\phi}(\x,\x_t)$ ~,\\
\STATE $\z_{t+1} = \argmin_{\z}~ g(\z) + \langle \y_t, \bA\x_{t+1} + \bB\z - \c \rangle + \frac{\rho}{2} \| \bA\x_{t+1} + \bB\z - \c \|^2$  ~,  \\
\STATE $\y_{t+1} = \y_t + \rho(\bA\x_{t+1} + \bB\z_{t+1} - \c)$ ~.
\STATE Receive a cost function $f_{t+1}$ and incur loss $f_{t+1}(\x_{t+1}) + g(\z_{t+1})$ and constraint violation $\|\bA\x_{t+1} + \bB\z_{t+1} - \c\|_2^2$;
\ENDFOR
\end{algorithmic}
\end{algorithm*}

For general convex functions, the following theorem shows that Algorithm \ref{alg:loadm1} achieves the $O(\sqrt{T})$ regret bounds, which is similar to OADM.
\begin{thm}\label{thm:loadm1}
Let the sequences $\{\x_t, \z_t,\y_t\}$ be generated by Algorithm \ref{alg:loadm1} and Assumption~\ref{asm:oadm} hold. For any $\x^*,\z^*$ satisfying $\bA\x^* + \bB\z^* = \c$, setting $\eta = \frac{G_f\sqrt{T}}{D_\x \sqrt{2\beta}}$ and $\rho = \sqrt{T}$,  we have
\begin{align}
&R_1(T)
\leq \frac{\lambda_{\max}^{\bB}D_{\z}^2\sqrt{T}}{2} + \frac{\sqrt{2}G_fD_\x\sqrt{T}}{\sqrt{\beta}} \label{eq:loadm1_bd} ~, \\
&R^c(T) \leq \lambda_{\max}^{\bB}D_\z^2 + \sqrt{2}D_{\x}G_f/\sqrt{\beta} + 2F\sqrt{T} \label{eq:loadm1_cst}~.
\end{align}
where $ 0 < \beta \leq  \alpha - \rho\lambda_{\max}^{\bA}/\eta$ and $\alpha$ is given in~\myref{eq:alpha}.
\end{thm}
\proof
Since $\x_{t+1}$ minimizes \myref{eq:oadm_x2}, we have
\begin{align}
- \{\bA^T\y_t + \rho\bA^T(\bA\x_{t} - \bB\z_t - \c)
&+ \eta(\nabla \phi(\x_{t+1}) - \nabla \phi(\x_t))\} \in \partial f_t(\x_{t+1})~.
\end{align}
%Following the similar derivation in \myref{eq:cf}, we have
%\begin{align}
%&f_t(\x_{t+1}) - f_t(\x^*) \nonumber \\
%& \leq -  \langle \bA^T\y_t + \rho  \bA^T(\bA\x_{t}+\bB\z_t - \c), \x_{t+1} - \x^*  \rangle  - \eta \langle \nabla \phi(\x_{t+1}) - \nabla \phi(\x_t), \x_{t+1} - \x^* \rangle \nonumber \\
%& = - \langle \y_t, \bA\x_{t+1} + \bB\z^* - \c \rangle +  \frac{\rho}{2}  ( \|\bB\z^* - \bB\z_t\|_2^2 -  \|\bA\x^* - \bA\x_{t}\|_2^2 - \|\bA\x_{t+1} + \bB\z_t - \c\|_2^2  \nonumber \\
%& + \| \bA\x_{t+1} - \bA\x_t \|_2^2 ) + \eta (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1}) - B_{\phi}(\x_{t+1} , \x_t)) ~.
%\end{align}
Following the similar derivation in lemma \ref{lem:bd1} yields
\begin{align}\label{eq:loadm1_bd1}
&f_t(\x_{t+1}) + g(\z_{t+1}) - (f_t(\x^*) + g(\z^*)) \nonumber \\
& \leq \frac{1}{2\rho}(\| \y_{t} \|_2^2 - \| \y_{t+1} \|_2^2)
- \frac{\rho}{2} \|\bA\x_{t+1} + \bB\z_t - \c\|_2^2 + \frac{\rho}{2}  ( \|\bB\z^* - \bB\z_t\|_2^2 -  \|\bB\z^* - \bB\z_{t+1}\|_2^2)  \nonumber \\
& +  \frac{\rho}{2}  ( \|\bA\x^* - \bA\x_{t+1}\|_2^2 -  \|\bA\x^* - \bA\x_{t}\|_2^2) + \eta (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1})) \nonumber \\
& + \frac{\rho}{2}\| \bA\x_{t+1} - \bA\x_t \|_2^2  - \eta B_{\phi}(\x_{t+1} , \x_t) ~.
\end{align}

Let $f_t'(\x_{t}) \in \partial f_t(\x_{t})$. Using the inequality $2 |\langle \x, \y \rangle| \leq \| \x\|_*^2 + \| \y \|^2$, we have
\begin{align}\label{eq:loadm1_f}
f_t(\x_{t}) - f_t(\x_{t+1}) & \leq \langle f_t'(\x_{t}), \x_t - \x_{t+1} \rangle =  \langle \frac{1}{\sqrt{\beta\eta}}f_t'(\x_{t}), \sqrt{\beta\eta} (\x_t - \x_{t+1}) \rangle \nonumber \\
& \leq \frac{1}{2\beta\eta} \| f_t'(\x_{t}) \|_*^2 + \frac{\beta\eta}{2} \|\x_t - \x_{t+1}\|^2 ~.
\end{align}
where $\beta > 0$.
Assume $ \beta \leq  \alpha - \rho\lambda_{\max}^{\bA}/\eta $ and $\alpha$ is in~\myref{eq:alpha}, we have
\begin{align}\label{eq:loadm1_fg}
&f_t(\x_{t}) + g(\z_{t+1}) - (f_t(\x^*) + g(\z^*)) \nonumber \\
& \leq \frac{1}{2\rho}(\| \y_{t} \|_2^2 - \| \y_{t+1} \|_2^2)
- \frac{\rho}{2} \|\bA\x_{t+1} + \bB\z_t - \c\|_2^2
+ \frac{\rho}{2}  ( \|\bB\z^* - \bB\z_t\|_2^2 -  \|\bB\z^* - \bB\z_{t+1}\|_2^2) \nonumber \\
& + \frac{1}{2\beta\eta} \| f_t'(\x_{t}) \|_*^2  +  \frac{\rho}{2}  ( \|\bA\x^* - \bA\x_{t+1}\|_2^2 -  \|\bA\x^* - \bA\x_{t}\|_2^2) + \eta (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1})) ~.
\end{align}

Summing over $t$ from $0$ to $T$, we have
\begin{align}
R_1(T)
& \leq  \frac{1}{2\rho}(\| \y_{0} \|_2^2 - \| \y_{T+1} \|_2^2)
+ \frac{\rho}{2}  ( \|\bB\z^* - \bB\z_0\|_2^2 -  \|\bB\z^* - \bB\z_{T+1}\|_2^2)  +\frac{1}{2\beta\eta} \sum_{t=0}^T \| f_t'(\x_{t}) \|_*^2 \nonumber \\
& +  \frac{\rho}{2}  ( \|\bA\x^* - \bA\x_{T+1}\|_2^2 -  \|\bA\x^* - \bA\x_{0}\|_2^2)
+ \eta (B_{\phi}(\x^*,\x_0) - B_{\phi}(\x^*, \x_{T+1}) ) \nonumber \\
& \leq \frac{\lambda_{\max}^{\bB}D_{\z}^2\rho}{2} + \eta D_{\x}^2 + \frac{G_f^2T}{2\beta \eta} ~.
\end{align}
Setting $\eta = \frac{G_f\sqrt{T}}{D_\x \sqrt{2\beta}}$ and $\rho = \sqrt{T}$ yields \myref{eq:loadm1_bd}.

Now we prove \myref{eq:loadm1_cst}. Rearranging the terms in \myref{eq:loadm1_bd1}, we have
\begin{align}
& \|\bA\x_{t+1} + \bB\z_t - \c\|_2^2 \leq \frac{2F}{\rho} + \frac{1}{\rho^2}(\| \y_{t} \|_2^2 - \| \y_{t+1} \|_2^2) +  ( \|\bB\z^* - \bB\z_t\|_2^2 -  \|\bB\z^* - \bB\z_{t+1}\|_2^2)  \nonumber \\
&+ \|\bA\x^* - \bA\x_{t+1}\|_2^2 -  \|\bA\x^* - \bA\x_{t}\|_2^2 + \frac{2\eta}{\rho} (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1})) ~.
\end{align}
Letting the assumptions hold and summing over $t$ from 0 to $T$, we have
\begin{align}\label{eq:loadm1_e}
& \sum_{t=0}^T \|\bA\x_{t+1} + \bB\z_t - \c\|_2^2 \nonumber \\
& \leq \frac{2FT}{\rho} + \frac{1}{\rho^2}(\| \y_{0} \|_2^2 - \| \y_{T+1} \|_2^2) +  ( \|\bB\z^* - \bB\z_0\|_2^2 -  \|\bB\z^* - \bB\z_{T+1}\|_2^2)  \nonumber \\
& + \|\bA\x^* - \bA\x_{T+1}\|_2^2 -  \|\bA\x^* - \bA\x_{0}\|_2^2 + \frac{2\eta}{\rho} (B_{\phi}(\x^*,\x_0) - B_{\phi}(\x^*, \x_{T+1})) \nonumber \\
& \leq \frac{2FT}{\rho} + \lambda_{\max}^{\bB}D_\z^2 + \frac{2\eta}{\rho}D_{\x}^2~.
\end{align}
Set $\eta = \frac{G_f\sqrt{T}}{D_\x \sqrt{2\beta}}$ and $\rho = \sqrt{T}$. According to Lemma \ref{lem:pdr}, we have \myref{eq:loadm1_cst}.
\qed

Similar to OADM, the regret bound for constraint violation could also reduced to a constant bound as in Theorem \ref{thm:cstbd} if additional assumptions on $\bB$ and subgradient of $g$ are satisfied. We do not prove it here, but it is easy to obtain the result by substituting $\rho$ and $\eta$ into the proof of Theorem \ref{thm:cstbd}.

If both $f_t$ and $g$ are strongly convex, we have the logarithmic regret bounds as established in the following theorem.
\begin{thm}\label{thm:loadm_logrgt}
Let Assumption~\ref{asm:oadm} hold. Assume $f_t(\x)$ and $g$ are respectively $\beta_1$- and $\beta_2$-strongly convex as in \myref{eq:fsc} and \myref{eq:gsc}. Setting $\eta_t = \beta_1 t, \rho_t = \beta_2 t/\lambda_{\max}^{\bB}$, we have
\begin{align}
& R_1(T) \leq \frac{G_f^2}{2\beta\beta_1} \log{(T+1)} + \frac{\beta_2 D_{\z}^2}{2} + \beta_1 D_{\x}^2~, \label{eq:loadm1_logrgt1} \\
&R^c(T) \leq \frac{2F\lambda_{\max}^{\bB}\log(T+1)}{\beta_2} + \lambda_{\max}^{\bB}D_\z^2 + \frac{2\beta_1\lambda_{\max}^{\bB}D_{\x}^2}{\beta_2} \label{eq:loadm1_logrgt2}~.
\end{align}
where $\alpha \geq \frac{\beta_2\lambda_{\max}^{\bA}}{\beta_1 \lambda_{\max}^{\bB}}$ and $0 < \beta \leq \alpha - \frac{\beta_2\lambda_{\max}^{\bA}}{\beta_1\lambda_{\max}^{\bB}}$ .
\end{thm}
\proof
 Replace $\rho,\eta$ by $\rho_t,\eta_t$ in~\myref{eq:loadm1_fg} in Theorem \ref{thm:loadm1}  and assume $\beta \eta_t + \rho_t \lambda_{\max}^{\bA} \leq \alpha \eta_t$.  Using the strong convexity of $f_t$ and $g$ and summing ~\myref{eq:loadm1_fg} over $t$ from $0$ to $T$, we have
\begin{align}
R_1(T) & \leq \sum_{t=0}^T  \frac{1}{2\rho_{t+1}}(\| \y_{t} \|_2^2 - \| \y_{t+1} \|_2^2) + \frac{1}{2\beta} \sum_{t=0}^T  \frac{1}{\eta_{t+1}}\| f_t'(\x_{t}) \|_2^2 \nonumber \\
& + \sum_{t=0}^T (\frac{\rho_{t+1}}{2}  ( \|\bB\z^* - \bB\z_t\|_2^2 -  \|\bB\z^* - \bB\z_{t+1}\|_2^2) - \frac{\beta_2}{2}\|\z^* - \z_{t+1}\|_2^2) \nonumber \\
& + \sum_{t=0}^T \frac{\rho_{t+1}}{2}  ( \|\bA\x^* - \bA\x_{t+1}\|_2^2 -  \|\bA\x^* - \bA\x_{t}\|_2^2) \nonumber \\
& + \sum_{t=0}^T (\eta_{t+1} (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1})) - \beta_1 B_{\phi}(\x^*, \x_{t+1}) )~.
\end{align}
Set $\rho_t = \beta_2 t/\lambda_{\max}^{\bB}$ and $\eta_t = \beta_1 t$. Therefore, $\beta \leq \alpha - \frac{\beta_2\lambda_{\max}^{\bA}}{\beta_1\lambda_{\max}^{\bB}}$, where $\alpha \geq \beta_2\lambda_{\max}^{\bA}/(\beta_1 \lambda_{\max}^{\bB})$.
Since $\rho_t$ is non-decreasing,
\begin{align}\label{eq:loadm1_Ax}
\sum_{t=0}^T \frac{\rho_{t+1}}{2}  ( \|\bA\x^* - \bA\x_{t+1}\|_2^2 -  \|\bA\x^* - \bA\x_{t}\|_2^2) \leq \frac{\rho_{T+1}}{2} \|\bA\x^* - \bA\x_{T+1}\|_2^2~,
\end{align}
The right-hand side can be canceled out by $-(\eta_{T+1}+\beta_1)B_{\phi}(\x^*,\x_{T+1})$ because $(\eta_{T+1}+\beta_1)\alpha \geq \rho_{T+1}\lambda_{\max}^{\bA}$.

Following the same derivation in~\myref{eq:yrho}-\myref{eq:logrgt_phi} in Theorem \ref{thm:oadm_logrgtbd1} yield the results.
\qed

%\begin{thm} Let assumptions (1)-(4) hold and $f_t(\x)$ be strongly convex defined in \myref{eq:fsc}. After $T$ rounds, we have
%\begin{align}
%& R_1(T) \leq \frac{G_f^2}{2\alpha\beta_1} \log{(T+1)} + \frac{\lambda_{\max}^{\bB}D_{\z}^2T^{1/4}}{2} + \beta_1 D_{\x}^2~. \label{eq:logrgt1} \\
%& R^c(T)\leq 2FT^{3/4} + \lambda_{\max}^{\bB}D_\z^2 + 2\beta_1D_{\x}^2T^{-1/4} \label{eq:logrgt1_cst}~.
%\end{align}
%\end{thm}
%\proof
%Assume that $f_t$ is $\beta_1$-strongly convex. Since $g$ is not assumed to be a strongly convex function, removing the term $-\frac{\beta_2}{2} \| \z^* - \z_{t+1} \|_2^2$ in \myref{eq:R1_logrgt} and using fixed $\rho$ yield
%\begin{align}
%R_1(T) & \leq \frac{1}{2\rho}(\| \y_{0} \|_2^2 - \| \y_{T+1} \|_2^2) + \frac{1}{2\alpha} \sum_{t=0}^T \frac{1}{\eta_{t+1}}\| f_t'(\x_{t}) \|_2^2 + \frac{\rho}{2}  ( \|\bB\z^* - \bB\z_0\|_2^2 -  \|\bB\z^* - \bB\z_{T+1}\|_2^2) \nonumber \\
%& + \sum_{t=0}^T (\eta_{t+1} (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1})) - \beta_1 B_{\phi}(\x^*, \x_{t+1}) )~.
%\end{align}
%Using \myref{eq:logrgt_phi} and setting $\eta_t = \beta_1 t$ yield
%\begin{align}
%& R_1(T) \leq \frac{G_f^2}{2\alpha} \sum_{t=0}^T \frac{1}{\beta_1 (t+1)} + \frac{\lambda_{\max}^{\bB}D_{\z}^2\rho}{2} +  \beta_1 D_{\x}^2~.
%\end{align}
%Applying $\sum_{t=0}^T \frac{1}{t+1} \leq \log(T+1)$ and setting $\rho = T^{1/4}$ give \myref{eq:logrgt1}.
%
%Now we prove \myref{eq:logrgt1_cst}. Using fixed $\rho$ in \myref{eq:log11_cstone}, we have
%\begin{align}
%\|\bA\x_{t+1} + \bB\z_t - \c\|_2^2 &\leq \frac{2F}{\rho} + \frac{1}{\rho^2}(\| \y_{t} \|_2^2 - \| \y_{t+1} \|_2^2) +  ( \|\bB\z^* - \bB\z_t\|_2^2 -  \|\bB\z^* - \bB\z_{t+1}\|_2^2)  \nonumber \\
%&+ \frac{2\eta_{t+1}}{\rho} (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1}) - \beta_1B_{\phi}(\x^*,\x_{t+1})) ~.
%\end{align}
%Letting the assumptions hold and summing over $t$ from 0 to $T$, we have
%\begin{align}
%\sum_{t=0}^T \|\bA\x_{t+1} + \bB\z_t - \c\|_2^2 & \leq \frac{2FT}{\rho} + \frac{1}{\rho^2}(\| \y_{0} \|_2^2 - \| \y_{T+1} \|_2^2)  +  ( \|\bB\z^* - \bB\z_0\|_2^2 -  \|\bB\z^* - \bB\z_{T+1}\|_2^2)  \nonumber \\
%&+ \sum_{t=0}^T\frac{2\eta_{t+1}}{\rho} (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1}) - \beta_1B_{\phi}(\x^*,\x_{t+1})) \nonumber \\
%& \leq \frac{2FT}{\rho} + \lambda_{\max}^{\bB}D_\z^2 + \frac{2\eta_1}{\rho}D_{\x}^2~.
%\end{align}
%Set $\eta_t = \beta_1 t$ and $\rho = T^{1/4}$. According to Lemma \ref{lem:pdr}, we have \myref{eq:logrgt1_cst}.
%\qed





==> loadm2.tex <==
\begin{algorithm*}[tb]
\caption{Online Inexact Alternating Direction Method 2 (OIADM2)}
\label{alg:loadm2}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} $f_{t+1}(\x) + g(\z), \bA,\bB,\c, \rho, \eta, \phi(\x)$
\STATE {\bfseries Initialization:} $\x_0,\z_0,\u_0 = \mathbf{0}$
\FOR{$t=0 \text{ to } T$}
\STATE $\x_{t+1} = \underset{\x}{\argmin}  \langle f_t'(\x_t) + \bA^T\{\y_t + \rho(\bA\x_t + \bB\z_t -\c)\}, \x - \x_t \rangle + \eta B_{\phi}(\x,\x_t)$ ~,\\
\STATE $\z_{t+1} = \argmin_{\z}~ g(\z) + \langle \y_t, \bA\x_{t+1} + \bB\z - \c \rangle + \frac{\rho}{2} \| \bA\x_{t+1} + \bB\z - \c \|^2$  ~,  \\
\STATE $\y_{t+1} = \y_t + \rho(\bA\x_{t+1} + \bB\z_{t+1} - \c)$ ~.
\STATE Receive a cost function $f_{t+1}$ and incur loss $f_{t+1}(\x_{t+1}) + g(\z_{t+1})$ and constraint violation $\|\bA\x_{t+1} + \bB\z_{t+1} - \c\|_2^2$;
\ENDFOR
\end{algorithmic}
\end{algorithm*}

If \myref{eq:oadm_x2} is still difficult to solve, but the gradient of $f_t$ is easy to compute, we can further linearize $f_t$ at $\x_t$ such that
\begin{align}\label{eq:oadm_x3}
\x_{t+1} = \underset{\x}{\argmin}  \langle f_t'(\x_t) + \bA^T\{\y_t + \rho(\bA\x_t + \bB\z_t -\c)\}, \x - \x_t \rangle + \eta B_{\phi}(\x,\x_t) ~.
\end{align}
In the batch setting, \myref{eq:oadm_x3} is known as inexact ADM~\cite{boyd10} if $\phi$ is a quadratic function. The OIADM2 is presented in Algorithm \ref{alg:loadm2}.

For general convex functions, Algorithm \ref{alg:loadm2} achieves the same regret bounds as Algorithm \ref{alg:loadm1}, which is shown in following theorem.
\begin{thm}\label{thm:loadm2}
Let the sequences $\{\x_t, \z_t,\y_t\}$ be generated by Algorithm \ref{alg:loadm2}. Let Assumption~\ref{asm:oadm} hold. For any $\x^*,\z^*$ satisfying $\bA\x^* + \bB\z^* = \c$, setting $\eta = \frac{G_f\sqrt{T}}{D_\x \sqrt{2\beta}}$ and $\rho = \sqrt{T}$,  we have
\begin{align}
&R_1(T)
\leq \frac{\lambda_{\max}^{\bB}D_{\z}^2\sqrt{T}}{2} + \frac{\sqrt{2}G_fD_\x\sqrt{T}}{\sqrt{\beta}} \label{eq:loadm2_bd} ~, \\
&R^c(T) \leq \lambda_{\max}^{\bB}D_\z^2 + \sqrt{2}D_{\x}G_f/\sqrt{\beta} + 2F\sqrt{T} \label{eq:loadm2_cst}~.
\end{align}
where $0 < \beta \leq \alpha - \rho\lambda_{\max}^{\bA}/\eta$ and $\alpha$ is given in~\myref{eq:alpha}.
\end{thm}
\proof
Since $\x_{t+1}$ minimizes \myref{eq:oadm_x2}, we have the following variational inequality:
\begin{align}
\langle f_t'(\x_{t}) + \bA^T \{\y_t + \rho\bA^T(\bA\x_{t} - \bB\z_t - \c)\}
+ \eta(\nabla \phi(\x_{t+1}) - \nabla \phi(\x_t)), \x_{t+1} - \x^*  \rangle \leq 0
\end{align}

%\begin{align}
%&f_t(\x_{t}) - f_t(\x^*) \nonumber \\
%& \leq -  \langle \bA^T\y_t + \rho  \bA^T(\bA\x_{t}+\bB\z_t - \c), \x_{t} - \x^*  \rangle  - \eta \langle \nabla \phi(\x_{t+1}) - \nabla \phi(\x_t), \x_{t} - \x^* \rangle \nonumber \\
%& = - \langle \y_t, \bA\x_{t} + \bB\z^* - \c \rangle +  \frac{\rho}{2}  ( \|\bB\z^* - \bB\z_t\|_2^2 -  \|\bA\x^* - \bA\x_{t}\|_2^2 - \|\bA\x_{t+1} + \bB\z_t - \c\|_2^2  \nonumber \\
%& + \| \bA\x_{t+1} - \bA\x_t \|_2^2 ) + \eta (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1}) - B_{\phi}(\x_{t+1} , \x_t)) ~.
%\end{align}

Rearranging the terms, we have
\begin{align}\label{eq:loadm2_fpt}
& \langle f_t'(\x_t), \x_{t+1} - \x^*\rangle \nonumber \\
& \leq -  \langle \bA^T\y_t + \rho  \bA^T(\bA\x_{t}+\bB\z_t - \c), \x_{t+1} - \x^*  \rangle  - \eta \langle \nabla \phi(\x_{t+1}) - \nabla \phi(\x_t), \x_{t+1} - \x^* \rangle \nonumber \\
& = - \langle \y_{t+1}, \bA\x_{t+1} + \bB\z^* - \c \rangle +  \frac{\rho}{2}  ( \|\bB\z^* - \bB\z_t\|_2^2 -  \|\bB\z^* - \bB\z_{t+1}\|_2^2 - \|\bA\x_{t+1} + \bB\z_t - \c\|_2^2  \nonumber \\
& + \| \bA\x_{t+1} + \bB\z_{t+1} - \c \|_2^2 ) + \eta (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1}) - B_{\phi}(\x_{t+1} , \x_t)) ~.
\end{align}

Letting $f_t'(\x_t) \in \partial f_t(\x_t)$, we have
\begin{align}\label{eq:loadm2_ft}
&f_t(\x_{t}) - f_t(\x^*) \leq \langle f_t'(\x_t), \x_t - \x^* \rangle = \langle f_t'(\x_t), \x_{t+1} - \x^*\rangle + \langle f_t'(\x_t), \x_t - \x_{t+1} \rangle~.
\end{align}

Assuming $ \beta \leq \alpha - \rho\lambda_{\max}^{\bA}/\eta$ and following the same derivation in~\myref{eq:loadm1_f}-\myref{eq:loadm1_e} in Theorem \ref{thm:loadm1} yields the results.
\qed

The $O(\sqrt{T})$ bound of constraint violation could also be reduced to a constant bound as in Theorem \ref{thm:cstbd} if additional assumptions on $\bB$ and subgradient of $g$ are satisfied. The following theorem shows Algorithm \ref{alg:loadm2} also achieves the logarithmic regret bounds for $R_1$ and $R^c$ when $f_t$ and $g$ are strongly convex.

\begin{thm}
Let assumptions (1)-(4) hold. Assume $f_t(\x)$ and $g$ are strongly convex given in \myref{eq:fsc} and \myref{eq:gsc}. Setting $\eta_t = \beta_1 t, \rho_t = \beta_2 t/\lambda_{\max}^{\bB}$, we have
\begin{align}
& R_1(T) \leq \frac{G_f^2}{2\beta\beta_1} \log{(T+1)} + \frac{\beta_2 D_{\z}^2}{2} + \beta_1 D_{\x}^2~, \label{eq:loadm1_logrgt1} \\
&R^c(T) \leq \frac{2F\lambda_{\max}^{\bB}\log(T+1)}{\beta_2} + \lambda_{\max}^{\bB}D_\z^2 + \frac{2\beta_1\lambda_{\max}^{\bB}D_{\x}^2}{\beta_2} \label{eq:loadm1_logrgt2}~.
\end{align}
where $\alpha \geq \frac{\beta_2\lambda_{\max}^{\bA}}{\beta_1 \lambda_{\max}^{\bB}}$ and $0 < \beta \leq \alpha - \frac{\beta_2\lambda_{\max}^{\bA}}{\beta_1\lambda_{\max}^{\bB}}$.
\end{thm}
\proof
Let $f_t'(\x_t) \in \partial f_t(\x_t)$. Using the strong convexity of $f_t$ and following the same derivation in~\myref{eq:loadm2_ft} in Theorem~\ref{thm:loadm2}, we have
\begin{align}
&f_t(\x_{t}) - f_t(\x^*) \leq \langle f_t'(\x_t), \x_{t+1} - \x^*\rangle + \langle f_t'(\x_t), \x_t - \x_{t+1} \rangle - \beta_1 B_{\phi}(\x^*,\x_t)~.
\end{align}

 Assume $\beta \eta_t + \rho_t \lambda_{\max}^{\bA} \leq \alpha \eta_t$ and recall~\myref{eq:loadm2_fpt}. Following the similar derivation in~\myref{eq:loadm1_f}-\myref{eq:loadm1_fg} in Theorem \ref{thm:loadm1}, using the strong convexity of $g$ and summing over $t$ from $0$ to $T$, we have
\begin{align}
R_1(T) & \leq \sum_{t=0}^T  \frac{1}{2\rho_{t+1}}(\| \y_{t} \|_2^2 - \| \y_{t+1} \|_2^2) + \frac{1}{2\beta} \sum_{t=0}^T  \frac{1}{\eta_{t+1}}\| f_t'(\x_{t}) \|_2^2 \nonumber \\
& + \sum_{t=0}^T (\frac{\rho_{t+1}}{2}  ( \|\bB\z^* - \bB\z_t\|_2^2 -  \|\bB\z^* - \bB\z_{t+1}\|_2^2) - \frac{\beta_2}{2}\|\z^* - \z_{t+1}\|_2^2) \nonumber \\
& + \sum_{t=0}^T \frac{\rho_{t+1}}{2}  ( \|\bA\x^* - \bA\x_{t+1}\|_2^2 -  \|\bA\x^* - \bA\x_{t}\|_2^2) \nonumber \\
& + \sum_{t=0}^T (\eta_{t+1} (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1})) - \beta_1 B_{\phi}(\x^*, \x_{t}) )~.
\end{align}
The telescoping sum of the last term is the same as~\myref{eq:logrgt_phi}, i.e.,
\begin{align}
&\sum_{t=0}^T (\eta_{t+1} (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1})) - \beta_1 B_{\phi}(\x^*, \x_{t}) ) \nonumber \\
& \leq \eta_1B_{\phi}(\x^*,\x_0) + \sum_{t=1}^T B_{\phi}(\x^*,\x_t)(\eta_{t+1} - \eta_{t} -\beta_1 )~.
\end{align}
Set $\rho_t = \beta_2 t/\lambda_{\max}^{\bB}$ and $\eta_t = \beta_1 t$, thus $\beta \leq \alpha - \frac{\beta_2\lambda_{\max}^{\bA}}{\beta_1\lambda_{\max}^{\bB}}$, where $\alpha \geq \beta_2\lambda_{\max}^{\bA}/(\beta_1 \lambda_{\max}^{\bB})$.
Using~\myref{eq:yrho}-\myref{eq:logrgt_z} in Theorem \ref{thm:oadm_logrgtbd1} and following the same derivation in~\myref{eq:loadm1_Ax} in Theorem~\ref{thm:loadm1} yield the results.
\qed

%Note $R^c$ also has a constant bound if Assumption~\ref{asm:oadmc} holds.
The regret bounds for OIADM2 can be converted to convergence rates in the stochastic setting based on the known online-stochastic conversion~\cite{Cesa04:stochastic,duchi09,xiao10}. More specifically, the stochastic convergence rates in expectation can be obtained by simply dividing regret bounds by $T$. Using martingale concentration results~\cite{Cesa04:stochastic,duchi09,xiao10}, the high probability bounds can also be obtained by applying the Azuma-Hoeffding inequality~\cite{azuma}.




==> pf_log1.tex <==

We consider the case that $f_t$ is strongly convex but $g$ is not strongly convex, e.g., $g$ is $\ell_1$ regularizer or an indicator function. This case includes some well-known examples we encounter in machine learning, e.g., generalized and group lasso~\citep{boyd10,Yuan06:grouplasso}.
We show that our algorithm can achieve $O(T^{1/4})$ regret bound for the objective. The regret bound for the constraint violation is $O(T^{3/4})$ but can be reduced to $\sqrt{T}$ given additional assumptions, which are satisfied in generalized and group lasso. Assume $f_t(\x)$ is $\beta_1$-strongly convex with respect to the function $\phi$, as given in \myref{eq:fsc}.

\begin{thm} \label{thm:oadmm1_rgtbd_strong}
Let the sequences $\{\x_t, \z_t,\y_t\}$ be generated by OADM. Let Assumption~\ref{asm:oadm} hold and $f_t(\x)$ be strongly convex defined in \myref{eq:fsc}. Set $\eta_t = \beta_1 t$. After $T$ rounds, we have
%\begin{align}
%& R_1(T) \leq \frac{G_f^2}{2\alpha\beta_1} \log{(T+1)} + \frac{\lambda_{\max}^{\bB}D_{\z}^2T^{1/4}}{2} + \beta_1 D_{\x}^2~, \label{eq:logrgt1} \\
%& R^c(T)\leq 2FT^{3/4} + \lambda_{\max}^{\bB}D_\z^2 + 2\beta_1D_{\x}^2T^{-1/4} \label{eq:logrgt1_cst}~.
%\end{align}
\begin{align}
& R_1(T) \leq \frac{G_f^2}{2\alpha\beta_1} \log{(T+1)} + \frac{\lambda_{\max}^{\bB}D_{\z}^2\rho}{2} +  \beta_1 D_{\x}^2~, \label{eq:logrgt1} \\
& R^c(T)\leq \frac{2FT}{\rho} + \lambda_{\max}^{\bB}D_\z^2 + \frac{2\eta_1}{\rho}D_{\x}^2 \label{eq:logrgt1_cst}~.
\end{align}
\end{thm}
\proof
Assume that $f_t$ is $\beta_1$-strongly convex. Since $g$ is not assumed to be a strongly convex function, removing the term $-\frac{\beta_2}{2} \| \z^* - \z_{t+1} \|_2^2$ in \myref{eq:R1_logrgt} and using fixed $\rho$ yield
\begin{align}
R_1(T) & \leq \frac{1}{2\rho}(\| \y_{1} \|_2^2 - \| \y_{T+1} \|_2^2) + \frac{1}{2\alpha} \sum_{t=1}^T \frac{1}{\eta_{t+1}}\| f_t'(\x_{t}) \|_*^2 + \frac{\rho}{2}  ( \|\bB\z^* - \bB\z_1\|_2^2 -  \|\bB\z^* - \bB\z_{T+1}\|_2^2) \nonumber \\
& + \sum_{t=1}^T (\eta_{t+1} (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1})) - \beta_1 B_{\phi}(\x^*, \x_{t+1}) )~.
\end{align}
Using \myref{eq:logrgt_phi} and setting $\eta_t = \beta_1 t$ yield
\begin{align}
& R_1(T) \leq \frac{G_f^2}{2\alpha} \sum_{t=0}^T \frac{1}{\beta_1 (t+1)} + \frac{\lambda_{\max}^{\bB}D_{\z}^2\rho}{2} +  \beta_1 D_{\x}^2~.
\end{align}
Applying $\sum_{t=1}^T \frac{1}{t+1} \leq \log(T+1)$ gives \myref{eq:logrgt1}.
%and setting $\rho = T^{1/4}$

Now we prove \myref{eq:logrgt1_cst}. Using fixed $\rho$ in \myref{eq:log11_cstone}, we have
\begin{align}
\|\bA\x_{t+1} + \bB\z_t - \c\|_2^2 &\leq \frac{2F}{\rho} + \frac{1}{\rho^2}(\| \y_{t} \|_2^2 - \| \y_{t+1} \|_2^2) +  ( \|\bB\z^* - \bB\z_t\|_2^2 -  \|\bB\z^* - \bB\z_{t+1}\|_2^2)  \nonumber \\
&+ \frac{2\eta_{t+1}}{\rho} (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1}) - \beta_1B_{\phi}(\x^*,\x_{t+1})) ~.
\end{align}
Letting Assumption~\ref{asm:oadm} hold and summing over $t$ from 0 to $T$, we have
\begin{align}
\sum_{t=1}^T \|\bA\x_{t+1} + \bB\z_t - \c\|_2^2 & \leq \frac{2FT}{\rho} + \frac{1}{\rho^2}(\| \y_{1} \|_2^2 - \| \y_{T+1} \|_2^2)  +  ( \|\bB\z^* - \bB\z_1\|_2^2 -  \|\bB\z^* - \bB\z_{T+1}\|_2^2)  \nonumber \\
&+ \sum_{t=1}^T\frac{2\eta_{t+1}}{\rho} (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1}) - \beta_1B_{\phi}(\x^*,\x_{t+1})) \nonumber \\
& \leq \frac{2FT}{\rho} + \lambda_{\max}^{\bB}D_\z^2 + \frac{2\eta_1}{\rho}D_{\x}^2~.
\end{align}
Set $\eta_t = \beta_1 t$. According to Lemma \ref{lem:pdr}, we have \myref{eq:logrgt1_cst}.
\qed

Setting $\rho = T^{\delta}$, we have $R_1(T) \leq O(T^\delta)$ and $R^c(T) \leq O(T^{1-\delta})$. In particular, if $\rho = T^{1/4}$, then $R_1(T) \leq O(T^{1/4})$ and $R^c(T) \leq O(T^{3/4})$. If Assumption~\ref{asm:oadmc} is further satisfied, we have a $O(\sqrt{T})$ regret bound for the constraints violation while the regret bound for the objective stays unchanged at $O(T^{1/4})$. .

\begin{thm}
Let the sequences $\{\x_t, \z_t,\y_t\}$ be generated by OADM and Assumption~\ref{asm:oadmc} be satisfied. Setting $\rho = T^{1/4}$, then
\begin{align}
&\sum_{t=1}^T \| \bA\x_{t+1} + \bB\z_{t+1} - \c \|_2^2 \leq 4D^2_\y\sqrt{T}~. \label{eq:oadmm1_logcst1}
\end{align}
\end{thm}
\proof
Setting $\rho = T^{1/4}$ in \myref{eq:cst111} gives \myref{eq:oadmm1_logcst1}.
\qed 

==> sadmwang.tex <==
Moving the term $\frac{\rho}{2} \|\bA\x_{t+1} + \bB\z_t - \c\|_2^2$  to the left hand side of \myref{eq:oadm1_r0}, we have 
\begin{align}
&f(\x_{t}) + g(\z_{t+1}) - (f_t(\x^*) + g(\z^*)) + \frac{\rho}{2} \|\bA\x_{t+1} + \bB\z_t - \c\|_2^2 \nonumber \\
& \leq \frac{1}{2\rho}(\| \y_{t} \|_2^2 - \| \y_{t+1} \|_2^2)
+ \frac{\rho}{2}  ( \|\bB\z^* - \bB\z_t\|_2^2 -  \|\bB\z^* - \bB\z_{t+1}\|_2^2) \nonumber \\
& \quad + \frac{1}{2\alpha\eta} \| f_t'(\x_{t}) \|_q^2  + \eta (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1})) ~.
\end{align}
Using Lemma \ref{lem:pdr},  we have
\begin{align}
&f(\x_{t}) + g(\z_{t+1}) - (f_t(\x^*) + g(\z^*)) + \frac{\rho}{2} \|\bA\x_{t+1} + \bB\z_{t+1} - \c\|_2^2 \nonumber \\
& \leq \frac{1}{2\rho}(\| \y_{t} \|_2^2 - \| \y_{t+1} \|_2^2)
+ \frac{\rho}{2}  ( \|\bB\z^* - \bB\z_t\|_2^2 -  \|\bB\z^* - \bB\z_{t+1}\|_2^2) \nonumber \\
& \quad + \frac{1}{2\alpha\eta} \| f_t'(\x_{t}) \|_q^2  + \eta (B_{\phi}(\x^*,\x_t) - B_{\phi}(\x^*, \x_{t+1})) ~.
\end{align}
